High-dimensional Bayesian Optimization of Hyperparameters for an Attention-based Network to Predict Materials Property: a Case Study on CrabNet using Ax and SAASBO

Expensive-to-train deep learning models can benefit from an optimization of the hyperparameters that determine the model architecture. We optimize 23 hyperparameters of a materials informatics model, Compositionally-Restricted Attention-Based Network (CrabNet), over 100 adaptive design iterations using two models within the Adaptive Experimentation (Ax) Platform. This includes a recently developed Bayesian optimization (BO) algorithm, sparse axis-aligned subspaces Bayesian optimization (SAASBO), which has shown exciting performance on high-dimensional optimization tasks. Using SAASBO to optimize CrabNet hyperparameters, we demonstrate a new state-of-the-art on the experimental band gap regression task within the materials informatics benchmarking platform, Matbench (~4.5% decrease in mean absolute error (MAE) relative to incumbent). Characteristics of the adaptive design scheme as well as feature importances are described for each of the Ax models. SAASBO has great potential to both improve existing surrogate models, as shown in this work, and in future work, to efficiently discover new, high-performing materials in high-dimensional materials science search spaces.

==> equations/cov.tex <==
\begin{equation} \label{eq:cov} 
	\left(
\begin{array}{cc}
 r & 0 \\
 0 & r \\
\end{array}
\right)
\end{equation}
where $\text{r}$ represents extracted \gls{densmap} radius.

==> equations/mvn.tex <==
\begin{equation} \label{eq:mvn} 
	e^{-\frac{1}{2} (X-\mu )\cdot \frac{1}{\Sigma }\cdot (X-\mu )}
\end{equation}
where $X$, $\mu$, $\Sigma$, and $\cdot$ represent \gls{densmap} embedding position at which to be evaluated, train or validation \gls{densmap} embedding position, covariance matrix, and matrix multiplication, respectively.

==> equations/score.tex <==
\begin{equation} \label{eq:score} 
	\frac{1}{w_E+w_p}\left(w_E E_{\text{scaled},i}+w_p p_{\text{scaled},i}\right)
\end{equation}
where $w_E$, $w_p$, $E_{\text{scaled},i}$, and $p_{\text{scaled},i}$ represent bulk modulus weight, proxy weight, robust-scaled predicted bulk modulus of the i-th validation point, and robust-scaled predicted uniqueness proxy of the i-th validation point, respectively.

==> equations/train-contrib-dens-2.tex <==
\begin{equation} \label{eq:train-contrib-dens} 
	\sum _{i=1}^{n_{\text{train}}} e^{-\frac{1}{2}\left(X_{v,j}-\mu _{t,i}\right)\cdot \frac{1}{\Sigma _{t,i}}\cdot \left(X_{v,j}-\mu _{t,i}\right)}
\end{equation}
where $X_{v,j}$, $\mu _{t,i}$, $\Sigma _{t,i}$, $\cdot$, and $n_{\text{train}}$ represent j-th validation \gls{densmap} embedding position at which to be evaluated, i-th train \gls{densmap} embedding position, i-th train covariance matrix, matrix multiplication, and total number of train points, respectively,

==> equations/train-contrib-dens.tex <==
\begin{equation} \label{eq:train-contrib-dens} 
	\sum _{i=1}^{n_{\text{train}}} e^{-\frac{1}{2}\left(X_{v,j}-\mu _{t,i}\right)\cdot \frac{1}{\Sigma _{t,i}}\cdot \left(X_{v,j}-\mu _{t,i}\right)}
\end{equation}
where $X_{v,j}$, $\mu _{t,i}$, $\Sigma _{t,i}$, $\cdot$, and $n_{\text{train}}$ represent j-th validation \gls{densmap} embedding position at which to be evaluated, i-th train \gls{densmap} embedding position, i-th train covariance matrix, matrix multiplication, and total number of train points, respectively.


==> equations/valid-frac.tex <==
\begin{equation} \label{eq:valid-frac} 
	f_k=\frac{n_{\text{val},k}}{n_{\text{val},k}+n_{\text{train},k}}
\end{equation}
where $f_k$, $n_{\text{val},k}$, and $n_{\text{train},k}$ represent validation fraction of the k-th cluster, number of validation points in the k-th cluster, and number of training points in the k-th cluster, respectively.

==> equations/weighted-rmse-2.tex <==
\begin{align}
\label{eq:weighted-rmse}
\begin{split}
	\frac{1}{w_E+w_p}\Biggl(w_E\sqrt{\frac{1}{n_{\text{val}}}\sum _{i=1}^{n_{\text{val}}} \left(E_{\text{true},i}-E_{\text{pred},i}\right){}^2} \\ 
	+ w_p\sqrt{\frac{1}{n_{\text{val}}}\sum _{i=1}^{n_{\text{val}}} \left(p_{\text{true},i}-p_{\text{pred},i}\right){}^2}\Biggr)
\end{split}
\end{align}
where $w_E$, $w_p$, $n_{\text{val}}$, $E_{\text{true},i}$, $E_{\text{pred},i}$, $p_{\text{true},i}$, and $p_{\text{pred},i}$ represent bulk modulus weight, proxy weight, number of validation points, \gls{dft}-calculated bulk modulus of the i-th validation point, predicted bulk modulus of the i-th validation point, true proxy property of the i-th validation point, and predicted proxy property of the i-th validation point, respectively.

==> equations/weighted-rmse.tex <==
\begin{widetext}
\begin{equation} \label{eq:weighted-rmse} 
	\frac{1}{w_E+w_p}\left(w_E\sqrt{\frac{1}{n_{\text{val}}}\sum _{i=1}^{n_{\text{val}}} \left(E_{\text{true},i}-E_{\text{pred},i}\right){}^2}+w_p\sqrt{\frac{1}{n_{\text{val}}}\sum _{i=1}^{n_{\text{val}}} \left(p_{\text{true},i}-p_{\text{pred},i}\right){}^2}\right)
\end{equation}
\end{widetext}
where $w_E$, $w_p$, $n_{\text{val}}$, $E_{\text{true},i}$, $E_{\text{pred},i}$, $p_{\text{true},i}$, and $p_{\text{pred},i}$ represent bulk modulus weight, proxy weight, number of validation points, \gls{dft}-calculated bulk modulus of the i-th validation point, predicted bulk modulus of the i-th validation point, true proxy property of the i-th validation point, and predicted proxy property of the i-th validation point, respectively.

==> latexmkrc <==
# Settings
$xdvipdfmx = "xdvipdfmx -z 6 -o %D %O %S";

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for sharelatex
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    $qpdf //= "/usr/local/bin/qpdf";
    $qpdf = $ENV{QPDF} if defined($ENV{QPDF}) && -x $ENV{QPDF};
    return if ! -x $qpdf; # check that qpdf exists
    $qpdf_opts //= "--linearize --newline-before-endstream";
    $qpdf_opts = $ENV{QPDF_OPTS} if defined($ENV{QPDF_OPTS});
    my $status = system($qpdf, split(' ', $qpdf_opts), "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
    system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
    $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
        system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
    if (-e $rtex_file) {
        do_knitr($rtex_file);
    }
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
    my $file = $_[0];
    my ($name, $path) = fileparse($file);
    pushd($path);
    my $return = system "mpost $name";
    popd();
    return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
        # change directory for a limited scope
        my $orig_dir = cwd();
        my $subdir = dirname($target);
        chdir($subdir);
        # run chktex on main file
        $status = system("/usr/bin/run-chktex.sh", $orig_dir, $file);
        # go back to original directory
        chdir($orig_dir);

        # in VALIDATE mode we always exit after running chktex
        # otherwise we exit if EXIT_ON_ERROR is set

        if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
            # chktex doesn't let us access the error info via exit status
            # so look through the output
            open(my $fh, "<", "output.chktex");
            my $errors = 0;
            {
                local $/ = "\n";
                while(<$fh>) {
                    if (/^\S+:\d+:\d+: Error:/) {
                        $errors++;
                        print;
                    }
                }
            }
            close($fh);
            exit(1) if $errors > 0;
            exit(0) if $ENV{'CHKTEX_VALIDATE'};
        }
    }
}

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

system("pdflatex main; pdflatex main; makeglossaries main; pdflatex main")

==> paper-pkgs.tex <==
\usepackage{auto-paper}

\PassOptionsToPackage{colorlinks}{hyperref}

\Crefname{figure}{Figure}{Figures} %needs to appear after hyperref and cleveref
\crefname{appsec}{Appendix}{Appendices}
\newcommand\crefrangeconjunction{--} % modify the reference style
\biboptions{sort&compress}

==> present-pkgs.tex <==
\usepackage{auto-paper}
\usepackage{adjustbox}
\usepackage{graphbox}

==> slides.tex <==
\section{Introduction} 
\subsection{Motivation}
\subsection{Prior Work}
\subsection{\glsentrytitlecase{vfzo}{long} Framework}
\section{Methods} 
\subsection{The \glsentrytitlecase{vfzo}{long} Framework}
%\subsubsection{Defining the \glsentrytitlecase{vfz}{long}}
%\subsubsection{Mapping \glsfmtshortpl{gb} to the \glsentrytitlecase{vfz}{long}}
%\subsubsection{Distance Calculations in the \glsentrytitlecase{vfz}{long}}
\subsection{Generating Random \glsentrytitlecase{vfzo}{long}s}
\subsection{Interpolation in the \glsentrytitlecase{vfzo}{long} Framework}
%\subsubsection{Barycentric Interpolation}
%\subsubsection{\glsentrytitlecase{gpr}{long}}
%\subsubsection{\glsentrytitlecase{idw}{long} Interpolation}
%\subsubsection{\glsentrytitlecase{nn}{long} Interpolation}
\subsection{Use of Interpolation Function}
\subsection{Literature Datasets}
%\subsubsection{\glsentrytitlecase{gpr}{long} for Fe Simulation Dataset}
%\subsubsection{\glsentrytitlecase{gpr}{long} for Ni Simulation Dataset}
%\subsubsection{\glsentrytitlecase{gprm}{long} for Fe Simulation Dataset}
\section{Results and Discussion} 
\subsection{Interpolation Accuracy}
%\subsubsection{Constant-Valued Control Models}
%\subsubsection{Experimental and Simulation Error}
%\subsubsection{Our Four Interpolation Methods}
%\subsubsection{Plotting \glsentrytitlecase{gbe}{long} between Arbitrary GBs}
\subsection{Interpolation Efficiency}
%\subsubsection{Comparison of Methods}
%\subsubsection{Symmetrization Runtime Comparison with Traditional Octonion Metric}
\subsection{Literature Datasets}
%\subsubsection{Comparison with Prior Work}
%\subsubsection{\glsentrytitlecase{gprm}{long} Applied to Fe Simulation Data}
\section{Conclusion} 
\section{Active vs. Passive Convention}
\section{Detailed Barycentric Interpolation Method}
\subsection{Triangulating a \glsentrytitlecase{vfz}{long} Mesh}
%\subsubsection{\glsentrytitlecase{svd}{long} Transformation from 8D Cartesian to 7D Cartesian}
%\subsubsection{Linearly Project onto Hyperplane}
%\subsubsection{\glsentrytitlecase{svd}{long} Transformation from 7D Cartesian to 6D Cartesian}
\subsection{Intersections in a \glsentrytitlecase{vfz}{long} Mesh}
%\subsubsection{Apply Same \glsentrytitlecase{svd}{long} to Input and Prediction Points}
%\subsubsection{Testing Nearby Facets for Intersections}
\subsection{Interpolation via Barycentric Coordinates}

